Slicenet: a Simple and Scalable Flow-Level Simulator for Network Slice Provisioning and Management

Network slicing plays a crucial role in the progression of 5G and beyond, facilitating dedicated logical networks to meet diverse and specific service requirements. The principle of End-to-End (E2E) slice includes not only a service chain of physical or virtual functions for the radio and core of 5G/6G networks but also the full path to the application servers that might be running at some edge computing or at central cloud. Nonetheless, the development and optimization of E2E network slice management systems necessitate a reliable simulation tool for evaluating different aspects at large-scale network topologies such as resource allocation and function placement models. This paper introduces Slicenet, a mininetlike simulator crafted for E2E network slicing experimentation at the flow level. Slicenet aims at facilitating the investigation of a wide range of slice optimization techniques, delivering measurable, reproducible results without the need for physical resources or complex integration tools. It provides a well-defined process for conducting experiments, which includes the creation and implementation of policies for various components such as edge and central cloud resources, network functions of multiple slices of different characteristics. Furthermore, Slicenet effortlessly produces meaningful visualizations from simulation results, aiding in comprehensive understanding. Utilizing Slicenet, service providers can derive invaluable insights into resource optimization, capacity planning, Quality of Service (QoS) assessment, cost optimization, performance comparison, risk mitigation, and Service Level Agreement (SLA) compliance, thereby fortifying network resource management and slice orchestration.

==> _extensions/mikemahoney218/arxiv/partials/_authors.tex <==
$-- You can use as many custom partials as you need. Convention is to prefix name with '_'
$-- It can be useful to use such template to split some template parts in smaller pieces, which is easier to reuse.
$-- This '_custom.tex' is used on 'title.tex' as example.
$-- See other existing format in quarto-journals/ organisation.
$-- %%%% TODO %%%%%
$-- Use it if you need to insert content at this specific place of the main Pandoc's template. Otherwise, remove it.
$-- Here we are using it to format the authors part of the template.
$-- %%%%%%%%%%%%%%%
\textbf{$it.name.literal$}$if(it.orcid)$~\orcidlink{$it.orcid$}$endif$$for(it.affiliations)$$it.department$\\$it.name$\\$if(it.city)$$it.city$$if(it.postal-code)$,\ $it.postal-code$$endif$$endif$$endfor$\\$if(it.email)$\href{mailto:$it.email$}{$it.email$}$endif$


==> _extensions/mikemahoney218/arxiv/partials/before-body.tex <==
$-- Implements the frontmatter, title page, and abstract.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, otherwise remove this partials to use Quarto default one
$-- %%%%%%%%%%%%%%%%
$if(has-frontmatter)$
\frontmatter
$endif$
$if(title)$
$if(beamer)$
\frame{\titlepage}
$else$
\maketitle
$endif$
$if(abstract)$
\begin{abstract}
$abstract$
\end{abstract}
$endif$
$endif$
$if(keywords)$
{\bfseries \emph Keywords}
\def\sep{\textbullet\ }
$for(keywords/allbutlast)$$keywords$ \sep $endfor$
$for(keywords/last)$$keywords$$endfor$

$endif$


==> _extensions/mikemahoney218/arxiv/partials/title.tex <==
$-- Provides configuration of document metadata for writing the title block.
$-- Note that in addition to these templates and partials, Quarto will also make normalized authors and affiliations data available to the template,
$-- making is easy to write custom title blocks against a standard schema.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, like below for printing the authors. Otherwise remove this partials to use Quarto default one.
$-- %%%%%%%%%%%%%%%%
$if(linenumbers)$
\usepackage{lineno}
\linenumbers
$endif$
$if(doublespacing)$
\usepackage{setspace}
\doublespacing
$endif$
$if(date)$
\renewcommand{\today}{$date$}
$endif$
\newcommand{\runninghead}{A Preprint }
$if(runninghead)$
\renewcommand{\runninghead}{$runninghead$ }
$endif$
$if(title)$
\title{$title$$if(thanks)$\thanks{$thanks$}$endif$}
$endif$
$if(subtitle)$
\usepackage{etoolbox}
\makeatletter
\providecommand{\subtitle}[1]{% add subtitle to \maketitle
  \apptocmd{\@title}{\par {\large #1 \par}}{}{}
}
\makeatother
\subtitle{$subtitle$}
$endif$
\def\asep{\\\\\\ } % default: all authors on same column
$if(authorcols)$
\def\asep{\And }
$endif$
\author{${ by-author:_authors.tex()[\asep] }}
\date{$date$}

